Information Transfer in Social Media

Recent research has explored the increasingly important role of social media by examining the dynamics of individual and group behavior, characterizing patterns of information diffusion, and identifying influential individuals. In this paper we suggest a measure of causal relationships between nodes based on the information-theoretic notion of transfer entropy, or information transfer. This theoretically grounded measure is based on dynamic information, captures fine-grain notions of influence, and admits a natural, predictive interpretation. Causal networks inferred by transfer entropy can differ significantly from static friendship networks because most friendship links are not useful for predicting future dynamics. We demonstrate through analysis of synthetic and real-world data that transfer entropy reveals meaningful hidden network structures. In addition to altering our notion of who is influential, transfer entropy allows us to differentiate between weak influence over large groups and strong influence over small groups.

==> ideas.tex <==
\subsection{Ideas}

From the BAA:
\begin{enumerate}
\item What are you trying to do?
\item How is it done today and what are the limitations?
\item Who will care and what will the impact be if you are successful?
\item How much will it cost, and how long will it take?
\end{enumerate}
The summary should include a description of the key technical challenges, a concise review of the technologies proposed to overcome these challenges and achieve the effortÕs goal, and a clear statement of the novelty and uniqueness of the proposed idea.


A deep understanding of dynamic networks requires us to go beyond simple considerations of static network structure. 
From the network perspective, a link is a link. But actually, we know from personal experience that some of our connections to fellow human beings are more important than others. Is it possible to identify the importance of a link just by looking at the dynamics of the agents? How much do the actions of one agent help us predict the actions of others. 

Current approaches consider static networks.
Or, dynamics assume the network structure itself is fixed, given, meaningful in some particular way.

If successful, our approach can deduce the true, hidden pattern significant connections underneath the apparent network. Essentially every network analysis tool we have would be enhanced by applying them to the ``true'' network rather than the apparent one. 


Information theory is an important approach to analyzing activity on networks.
\begin{enumerate}
\item The approach is model-free.
\item Rigorously quantifies the predictive power.
\item Fully takes advantage of dynamics
\item (I.T.) is asymmetric
\item Fine-grained, i.e., local information
\end{enumerate}

Challenges:
\begin{enumerate}
\item Requires lots of data.
\item Multi-timescale approaches must be developed.
\item Analysis is local, need connection with global measures
\end{enumerate}



==> sec-results-digg.tex <==

\subsection{Digg data}\label{sec:digg}
Digg is a popular social news portal that relies on users to submit
and moderate news stories. Each new story is added to an upcoming stories queue. Users express their interest in a story by {\em digging}, or voting, for that story. Digg's automatic  promotion algorithm looks at the voting patterns made within 24 hours of a story's submission. Of the thousands of stories submitted every day about a hundred are promoted and then displayed on the front page. 

Digg also allows users to designate friends and track their activities. The \emph{friends interface} shows  stories a user's friends recently submitted or voted for. The friendship graph is directed. When user $j$ lists user $i$ as a \emph{friend}, $j$ can watch the activities of $i$ but not vice versa. We call $j$ the \emph{fan}, or the follower, of $i$. A newly submitted story is visible in the upcoming stories list, as well as to submitter's fans through the friends interface. With each vote it also becomes visible to voter's fans.

Our dataset consists of information about 3,553 stories promoted to the front page in June 2009.\footnote{The data set is available at\\http://www.isi.edu/\textasciitilde lerman/downloads/digg2009.html} 
%
The data associated with each story contains story title, story id, link,  submitter's name, submission time, list of voters and the time of each vote, the time the story was promoted to the front page. We also have the network of (directed) friend relationships among the voters in our dataset.
There were 139,409 active users, of which 71,367 designated at least one other user as a friend. 

We look at the timing of votes for each active user. For a given user, this signal consists of a series of timestamps $(\tau_0, \tau_1,\ldots)$, denoting each time they voted. In the simplest approach to calculating information transfer, we discretize time into $M$ equal intervals labeled with $t = 1,\ldots,M$. Then $X_t = 1$ means that the user voted during the $t$-th time interval, while $X_t = 0$ if no vote occurred in that interval. Our dataset consists of about thirty days of activity split into bins of length 4 hours each. The choice of bin size depends on the amount of data available and will be discussed later.

For each pair of nodes $X,Y$ who had a directed edge, $X \rightarrow Y$, we calculated the information transfer, $T_{X\rightarrow Y}$ as in Eq.~\ref{eq:TE}.  In that equation we choose $k=l=7$. Based on a bin size of 4 hours, this implies that we are looking at activity in the past 28 hours to predict $Y$'s current activity. Looking at activity in this time range is based on empirical results about activity on Digg\cite{Lerman10icwsm}. 
The choice of bin width and number of bins is chosen according to the amount of data. 
In particular, if we calculate entropies based on $n$ bins of history, there are $2^n$ possible histories. In order to sample all possible histories we require that the total number of time bins is $\mathcal{O}(2^n)$. 

To validateÉ

\begin{figure*}[!h]
\centering
    \includegraphics[width=0.4\textwidth]{figs/Digg_validation2.png} \label{fig_validate}
     \caption{We compare the number of stories passed from user $X$ to user $Y$ with the information transfer $T_{X\rightarrow Y}$ calculated using only the timing. }
     \label{fig_0}
\end{figure*}


\begin{figure*}[!h]
\centering
\subfigure[]{
    \includegraphics[width=0.4\textwidth]{figs/topusers2} \label{fig_v}
    } %\hspace*{1cm}
    \subfigure[]{
    \includegraphics[width=0.4\textwidth]{figs/topuserstopedges3.pdf} \label{fig_c}
    }
   
     \caption{(a) Digg follower graph; (b) Transfer--entropy induced graph. }
     \label{fig_0}
\end{figure*}

\begin{figure*}[!h]
\centering
\subfigure[]{
    \includegraphics[width=0.4\textwidth]{figs/Digg_validation2} \label{fig:digg_validation}
    } %\hspace*{1cm}
     \caption{Digg validation}
     \label{fig_0}
\end{figure*}


